Bayesian Synthesis of Probabilistic Programs for Automatic Data Modeling

We present new techniques for automatically constructing probabilistic programs for data analysis, interpretation, and prediction. These techniques work with probabilistic domain-specific data modeling languages that capture key properties of a broad class of data generating processes, using Bayesian inference to synthesize probabilistic programs in these modeling languages given observed data. We provide a precise formulation of Bayesian synthesis for automatic data modeling that identifies sufficient conditions for the resulting synthesis procedure to be sound. We also derive a general class of synthesis algorithms for domain-specific languages specified by probabilistic context-free grammars and establish the soundness of our approach for these languages. We apply the techniques to automatically synthesize probabilistic programs for time series data and multivariate tabular data. We show how to analyze the structure of the synthesized programs to compute, for key qualitative properties of interest, the probability that the underlying data generating process exhibits each of these properties. Second, we translate probabilistic programs in the domain-specific language into probabilistic programs in Venture, a general-purpose probabilistic programming system. The translated Venture programs are then executed to obtain predictions of new time series data and new multivariate data records. Experimental results show that our techniques can accurately infer qualitative structure in multiple real-world data sets and outperform standard data analysis methods in forecasting and predicting new data.

==> Makefile <==
.PHONY:all
all: clean paper supplement zipup

paper:
	pdflatex paper
	bibtex paper
	pdflatex paper
	pdflatex paper

supplement:
	pdflatex supplement
	bibtex supplement
	pdflatex supplement
	pdflatex supplement
	zip supplement.zip supplement.pdf

.PHONY:slides
slides:
	pdflatex slides
	pdflatex slides

SERVER=probcomp.csail.mit.edu:/afs/csail/proj/probcomp/www/data/popl2019

.PHONY:deploy
deploy:
	scp paper.pdf ${SERVER}/popl184.pdf; \
	scp supplement.pdf ${SERVER}/popl184-supplement.pdf

.PHONY:zipup
zipup:
	zip popl184-tex.zip \
		abstract.sh \
		abstract.tex \
		acmart.cls \
		ACM-Reference-Format.bst \
		assets \
		css-xml.sh \
		conclusion.tex \
		dsllisting.tex \
		example.tex \
		experiments.tex \
		figures \
		introduction.tex \
		kbordermatrix.sty \
		languages.tex \
		Makefile \
		paper.bib \
		paper.pdf \
		paper.tex \
		preamble.tex \
		README \
		related.tex \
		semantics.tex \
		supplement.pdf \
		technical.tex \
		vslisting.tex

.PHONY:arxiv
arxiv: paper
	tar -cv \
		abstract.sh \
		abstract.tex \
		acmart.cls \
		ACM-Reference-Format.bst \
		assets \
		css-xml.sh \
		conclusion.tex \
		dsllisting.tex \
		example.tex \
		experiments.tex \
		figures \
		introduction.tex \
		kbordermatrix.sty \
		languages.tex \
		Makefile \
		paper.bib \
		paper.bbl \
		paper.tex \
		preamble.tex \
		README \
		related.tex \
		semantics.tex \
		supplement.tex \
		technical.tex \
		vslisting.tex > arxiv.tar.gz

.PHONY:clean
clean:
	-rm -f *.out *.aux  *.bbl  *.log  *.bcf  \
		*.blg  *.log  *.xml  *.toc  *.gz  *.out  *.fls  *.fdb_latexmk  \
		*.snm *.nav \
		paper.pdf supplement.pdf slides.pdf popl184-tex.zip


==> assets/evaluator <==
type NonTerminal = String
type Terminal = String
type Tag = String

type NonTerminals = Set [NonTerminal]
type Terminals = Set [Terminal]

nonterminals :: Set [NonTerminal]
nonterminals = Data.Set.fromList $ Prelude.map (\x-> "N" ++ show x) [1..10]

terminals :: Set [Terminal]
nonterminals = Data.Set.fromList $ Prelude.map (\x-> "s" ++ show x) [1..10]

Rewrite(Ni, Rik) = match Rik with
    | (Ni, tik, []) ->
        let s ~ Q(\tik, .)
        in (tik, s)
    | (Ni, tik, M_1 ... M_n) ->
        (tik, M...M)
    | otherwise -> fail

Expand(N_i) =
    let Rik ~ Discrete{(R'_{ik}, t'_{ik}) | k=1,2,\dots,r_i}
    in let N' = rewrite(Ni, Rik)
    in match N' with
        | (tik, s) -> (tik s), P(\tik)*Q(\tik, s)
        | (tik, M1...Mn) -> (tik Expand[M1] ... Expand[Mn]), P(\tik) \prod Pmi

def rewrite(Ni, Rik):
    match Rik with
        (Ni, tik, []) ->
            simulate s ~ Q(\tik, .)
            return (tik, s)
        (Ni, tik, Ns)
            return (tik, Ns)

def evaluate(S):
    sample \tik ~ P(S)
    S' = rewrite(S, Rik)
    match S' with
        | (tik, s) -> (tik, s)
        | (tik, Ns)
            -> return (tik, map(evaluate, Ns))


==> figures/crosscat-datasets.tex <==
%!TEX root = ../paper.tex

\begin{figure}

\footnotesize
\begin{subtable}[t]{.3\linewidth}
\caption{automobiles dataset}
\begin{tabular}{ll}
variable & stattype \\ \midrule
symboling & nominal \\
normalized-losses & numerical \\
make & nominal \\
fuel-type & nominal \\
aspiration & nominal \\
num-of-doors & nominal \\
body-style & nominal \\
drive-wheels & nominal \\
engine-location & nominal \\
wheel-base & numerical \\
length & numerical \\
width & numerical \\
height & numerical \\
curb-weight & numerical \\
engine-type & nominal \\
num-of-cylinders & nominal \\
engine-size & numerical \\
fuel-system & nominal \\
bore & numerical \\
stroke & numerical \\
compression-ratio & numerical \\
horsepower & numerical \\
peak-rpm & numerical \\
city-mpg & numerical \\
highway-mpg & numerical \\
price & numerical
\end{tabular}
\end{subtable}%
\begin{subtable}[t]{.3\linewidth}
\footnotesize
\caption{disease dataset}
\begin{tabular}{ll}
variable & stattype \\ \midrule
age & numerical \\
sex & nominal \\
chest-pain & nominal \\
resting-blood-pressure & numerical \\
cholesterol & numerical \\
fasting-blood-sugar & nominal \\
resting-electrocardiography & nominal \\
max-heart-rate & numerical \\
exercise-induced-angina & nominal \\
st-depression & numerical \\
slope-exercise & nominal \\
num-vessels-flourosopy & nominal \\
thal & nominal \\
disease & nominal \\
\end{tabular}
\end{subtable}\hfill%
\begin{subtable}[t]{.3\linewidth}
\caption{hepatitis dataset}
\begin{tabular}{ll}
variable & stattype \\ \midrule
class & nominal \\
age & numerical \\
sex & nominal \\
steroid & nominal \\
antivirals & nominal \\
fatigue & nominal \\
maliase & nominal \\
anorexia & nominal \\
liver-big & nominal \\
liver-firm & nominal \\
spleen-palpable & nominal \\
spiders & nominal \\
ascites & nominal \\
varices & nominal \\
bilirubin & numerical \\
alk-phosphate & numerical \\
sgot & numerical \\
albumin & numerical \\
protime & numerical \\
histology & nominal \\
\end{tabular}
\end{subtable}

\begin{subtable}[t]{.4\linewidth}
\caption{wine dataset}
\begin{tabular}{ll}
variable & stattype \\ \midrule
cultivar & nominal  \\
alcohol & numerical  \\
malic-acid & numerical  \\
ash & numerical  \\
alcalinity-of-ash & numerical  \\
magnesium & numerical  \\
total-phenols & numerical  \\
flavanoids & numerical  \\
nonflavanoid-phenols & numerical  \\
proanthocyanins & numerical  \\
color-intensity & numerical  \\
hue & numerical  \\
od280-od315-of-diluted-wines & numerical  \\
proline & numerical  \\
\end{tabular}
\end{subtable}\hfill%
\begin{subtable}[t]{.2\linewidth}
\footnotesize
\caption{credit dataset}
\begin{tabular}{ll}
variable & stattype \\ \midrule
A01 & nominal \\
A02 & numerical \\
A03 & numerical \\
A04 & nominal \\
A05 & nominal \\
A06 & nominal \\
A07 & numerical \\
A08 & nominal \\
A09 & nominal \\
A10 & numerical \\
A11 & nominal \\
A12 & nominal \\
A13 & numerical \\
A14 & numerical \\
A15 & nominal \\
\end{tabular}
\end{subtable}\hfill%
\begin{subtable}[t]{.3\linewidth}
\caption{census dataset}
\begin{tabular}{ll}
variable & stattype \\ \midrule
age & numerical \\
workclass & nominal \\
fnlwgt & numerical \\
education & nominal \\
education-num & numerical \\
marital-status & nominal \\
occupation & nominal \\
relationship & nominal \\
race & nominal \\
sex & nominal \\
capital-gain & numerical \\
capital-loss & numerical \\
hours-per-week & numerical \\
native-country & nominal \\
income & nominal \\
\end{tabular}
\end{subtable}

\caption{}
\label{fig:crosscat-datasets}
\end{figure}


==> figures/crosscat-notations.tex <==
%!TEX root = ../paper.tex

\begin{figure}

\footnotesize

\begin{subtable}[t]{.485\linewidth}
\footnotesize
\caption{DSL for CrossCat distributions and dependencies}
\label{subfig:crosscat-description-dsl-grammar}
\hrule
\begin{flalign*}
\tlar{distribution}     &=
    \mathsf{NIGNormal}\;
        \lar{h}_{\in \mathbb{R}}\;
        \lar{h}_{\in \mathbb{R}}\;
        \lar{h}_{\in \mathbb{R}}\;
        \lar{h}_{\in \mathbb{R}}\; \\
    &\; |\; \mathsf{GammaPoisson}\; \lar{h}_{\in \mathbb{R}}\; \\
    &\; |\; \mathsf{DirichletCategorical}\; \tlar{size}_{\in \mathbb{N}}\;
        \lar{h}_{\in \mathbb{R}} \\
\tlar{primitive}  &=
    \tlar{index}_{\in \mathbb{N}} \tlar{distribution} \\
\tlar{primitives} &=
    \tlar{primitive} | \tlar{primitives}, \tlar{primitive} \\
\tlar{block}         &=
    \tlar{concentration}_{\in\mathbb{R}} \tlar{primitives} \\
\tlar{blocks}        &=
    \tlar{block} | \tlar{blocks}, \tlar{block} \\
\tlar{program}       &=
    \tlar{blocks}
\end{flalign*}
\hrule
\end{subtable}\hfill%
\begin{subtable}[t]{.5\linewidth}
\caption{Symbols to describe prior and generative process}
\label{subfig:crosscat-description-symbols}
\begin{tabularx}{\linewidth}{|l|X|}
\hline
\textbf{Symbol} & \textbf{Description} \\ \hline
$\alpha_0$ & Concentration hyperparameter of column CRP \\
$\alpha_k$ & Concentration hyperparameter of row CRPs \\
$v_c$ & Block index of variable $c$ in column partition\\
$K$ & Number of blocks in col. partition, $\max{\bv}_{1:C}$\\
$\mt{V}^k$ & List of variables in block $k$ of col. partition \\
$z^k_r$ & Cluster index of $r$ in row partition of block $k$ \\
$\mt{C}^k_j$ & List of rows in cluster $j$ of block $k$ \\
$M_c$ & Primitive distribution of data for variable $c$ \\
$\lambda_c$ & Hyperparameters of $M_c$ \\
$Y_{[r,c]}$ & $r$-{th} observation of variable $c$ \\
\hline
\end{tabularx}
\end{subtable}

\bigskip

\begin{subtable}[t]{.4855\linewidth}
\caption{Prior $\mt{A}$ over DSL programs $\mt{S}_d$}
\label{subfig:crosscat-description-dsl-prior}
\begin{tabular*}{\linewidth}{ll}
\toprule
\multicolumn{2}{@{}l}{1. Sample column partition into blocks.} \\[3pt]
$\bv = (v_1,\dots,v_C) \sim \textsc{\small Crp}(\cdot; \alpha_0)$
  & \\
$\mt{V}^k \gets \set{c\,{\in}\,[C]: v_c\,{=}\,k}$
  & for $k=1\dotsc{K}$
  \\[3pt]
%
\multicolumn{2}{@{}l}{2. Sample column hyperparameters from hyperprior.} \\[3pt]
$\lambda_c \sim V_c$
    & for $c=1\dots{C}$
    \\[3pt]
%
\multicolumn{2}{@{}l}{3. Sample CRP concentration parameters.} \\[3pt]
$\alpha_k \sim \mathsf{Gamma}(1,1)$
    & for $k=1\dotsc{K}$
    \\[8pt] \bottomrule
\end{tabular*}
\end{subtable}
\begin{subtable}[t]{.475\linewidth}
\caption{Generative process for probabilistic program $\mt{S}_p$}
\label{subfig:crosscat-description-process}
\begin{tabular*}{\linewidth}{ll}
\toprule
\multicolumn{2}{@{}l}{1. Sample row partitions within each block.} \\[3pt]
$\bz^k\,{=}\,(z^k_1,\dots,z^k_N) \sim \textsc{\small Crp}(\cdot; \alpha_k)$
  & for $k=1\dotsc{K}$
  \\
$\mt{C}^k_j \gets \set{r\,{\in}\,[N]: z^k_r\,{=}\,j}$
  & for $k=1\dotsc{K}$
  \\
$\phantom{!}$
  & for $j=1\dotsc{\max\bz^k}$
  \\[3pt]
\multicolumn{2}{@{}l} {2. Sample data jointly within row cluster.} \\[3pt]
$\set{Y_{[r,c]} : r \in \mt{C}^k_j} \sim M_c(\cdot; \lambda_c)$
  & for $k=1\dotsc{K}$
  \\
$\phantom{!}$
  & for $j=1\dotsc{\max\bz^k}$
  \\
$\phantom{!}$
 & \;\; for $c\,{\in}\,\mt{V}^k$ \\ \bottomrule
\end{tabular*}
\end{subtable}
\captionsetup{skip=5pt}
\caption{DSL grammar, notations, prior, and generative process for a broad
class of probabilistic programs that model multivariate tabular data using
nonparametric Bayesian mixtures.}
\label{fig:crosscat-description}
\end{figure}


==> figures/crosscat-tutorial.tex <==
%!TEX root = ../paper.tex

\begin{figure}[ht]
\centering

\begin{subtable}[b]{\textwidth}
\tiny
\caption{Observed data records of patients in a heart disease study.}
\label{subfig:crosscat-synthesis-data}
\begin{tabular}{llllllllllllll}
\toprule
\multirow{2}{*}{age} & \multirow{2}{*}{sex} & \multirow{2}{*}{chest pain} & blood    & chol-    & blood    & electro     & heart    & exercise & ST       & slope    & vessels    & \multirow{2}{*}{thal} & \multirow{2}{*}{disease} \\
                     &                      &                             & pressure & estrol   & sugar    & cardiog.    & rate     & angina   & dep.     & exercise & fluoro.    &                       & \\ \midrule
63                   & M                    & typical angina              & 145      & 233      & >120     & hypertrophy & 150      & N        & 2.3      & down     & 0          & fixed                 & 0 \\
67                   & M                    & asymptomatic                & 160      & 286      & <120     & hypertrophy & 108      & Y        & 1.5      & flat     & 3          & normal                & 2 \\
67                   & M                    & asymptomatic                & 120      & 229      & <120     & hypertrophy & 129      & Y        & 2.6      & flat     & 2          & reversible            & 1 \\
37                   & M                    & non-anginal                 & 130      & 250      & <120     & normal      & 187      & N        & 3.5      & down     & 0          & fixed                 & 0 \\
41                   & F                    & atypical angina             & 130      & 204      & <120     & hypertrophy & 172      & N        & 1.4      & up       & 0          & fixed                 & 0 \\
62                   & F                    & asymptomatic                & 140      & 268      & <120     & hypertrophy & 160      & N        & 3.6      & down     & 2          & fixed                 & 3 \\
57                   & F                    & asymptomatic                & 120      & 354      & <120     & normal      & 163      & Y        & 0.6      & up       & 0          & fixed                 & 0 \\
38                   & M                    & non-anginal                 & 138      & 175      & <120     & normal      & 173.0    & N        & 0.0      & down     & ?          & reversible            & 0 \\
$\cdots$             & $\cdots$             & $\cdots$                    & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$    & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$ & $\cdots$   & $\cdots$              & $\cdots$ \\
\bottomrule
\end{tabular}
\end{subtable}
\bigskip

\begin{subfigure}[b]{\linewidth}
\begin{lstlisting}[style=venturescript,frame=single]
assume variable_to_block_assignment = dict(
  // Variables in block 0.
  ["chest-pain",0]          , ["max-heart-rate",0]         , ["exercise-induced-angina",0]   , ["thal",0]
  ["st-depression",0]       , ["slope-exercise",0]         , ["num-vessels-fluoroscopy",0]   , ["disease",0]
  // Variables in block 1.
  ["sex",1]                 ,["resting-blood-pressure",1]  , ["resting-electrocardiography",1],
  ["fasting-blood-sugar",1] ,["cholesterol",1]             , ["age",1]
);
assume variable_to_distributions = dict(
  // Mixture models in block 0.
  ["chest-pain",                  mem((cluster_idx) -> {make_symm_dirichlet_categorical(4, 1.)})],
  ["max-heart-rate",              mem((cluster_idx) -> {make_nig_normal(150.72, 1.78, 8114.99, 26.91)})],
  ["exercise-induced-angina",     mem((cluster_idx) -> {make_symm_dirichlet_categorical(2, 1.)})],
  ["st-depression",               mem((cluster_idx) -> {make_nig_normal(0.77, 0.04, 3.74, 15.05)})],
  ["slope-exercise",              mem((cluster_idx) -> {make_symm_dirichlet_categorical(3, 1.21)})],
  ["num-vessels-fluoroscopy",     mem((cluster_idx) -> {make_symm_dirichlet_categorical(4, 1.21)})],
  ["thal",                        mem((cluster_idx) -> {make_symm_dirichlet_categorical(3, 1.21)})],
  ["disease",                     mem((cluster_idx) -> {make_symm_dirichlet_categorical(5, 1.21)})],
  // Mixture models in block 1.
  ["age",                         mem((cluster_idx) -> {make_nig_normal(56.41, 1.78, 362.45, 6.93)})],
  ["sex",                         mem((cluster_idx) -> {make_symm_dirichlet_categorical(2, 3.87)})],
  ["resting-blood-pressure",      mem((cluster_idx) -> {make_nig_normal(136.10, 1.78, 1883.71, 8.41)})],
  ["cholesterol",                 mem((cluster_idx) -> {make_nig_normal(446.79, 0.02, 14063.83, 3.87)})],
  ["fasting-blood-sugar",         mem((cluster_idx) -> {make_symm_dirichlet_categorical(2, 1.)})],
  ["resting-electrocardiography", mem((cluster_idx) -> {make_symm_dirichlet_categorical(3, 1.)})]
);
assume block_to_mixture_weights = dict(
  [0,  simplex(0.3613, 0.3139, 0.2701, 0.0328, 0.0219)],
  [1,  simplex(0.6460, 0.3504, 0.0036)]
);
assume get_row_mixture_assignment = mem((rowid, block) ~> {
    weights = block_to_mixture_weights[block];
    categorical(weights) #mixture_assignment:pair(rowid, block)
});
assume get_cell_value = (rowid, variable) ~> {
    block = variable_to_block_assignment[variable];
    row_mixture_assignment = get_row_mixture_assignment(rowid, block);
    sampler = variable_to_distributions[variable](row_mixture_assignment);
    sampler() #cell_value:pair(rowid, variable)
};
\end{lstlisting}
\captionsetup{skip=0pt}
\caption{Synthesized probabilistic model program representing generative model
    for cells in the table.}
\label{subfig:crosscat-synthesis-code}
\end{subfigure}

\begin{subfigure}[b]{\linewidth}
\begin{lstlisting}[style=venturescript,frame=single]
define id_new_patient = -1;
observe get_cell_value(id_new_patient, variable: "chest-pain") = 2
observe get_cell_value(id_new_patient, variable: "cholesterol") = 160
for_each(["chest-pain", "cholesterol"], (variable) -> {
    block = run(sample(variable_to_block_assignment[${variable}]));
    mh([|mixture_assignment|], pair(id_new_patitent, block), one, steps:10)});
mapM((variable) -> {predict get_cell_value(${id_new_patient}, ${variable})}, ["thal", "age", "disease"])
// [0, 52.29076185834388, 1]
\end{lstlisting}
\captionsetup{skip=0pt}
\caption{Executing the synthesized program in the Venture inference engine to
  formulate joint predictions on a new partially-observed patient data record.}
\label{subfig:crosscat-synthesis-analysis}
\end{subfigure}
\captionsetup{skip=5pt}
\caption{Synthesized probabilistic program given observations in a tabular dataset.}
\label{fig:crosscat-synthesis}
\end{figure}


==> figures/diagram.tex <==
%!TEX root = ../paper.tex

\begin{figure}[!htb]

\footnotesize

\begin{tikzpicture}[thick]

\node[
    rectangle,
    draw=black,
    minimum height=2.15cm,
    text width=8.25cm,
    align=center,
] (synthesis-system) {};

\node[
    rectangle,
    draw=black,
    above=0 of synthesis-system.north,
    align=center,
    anchor=south,
    text width=8.25cm,
] (system-title) {Bayesian Probabilistic Program Synthesis System};

\node[
    rectangle,
    draw=black,
    text width=2.5cm,
    minimum height=.9cm,
    align=center,
    % left=.85 of system-title.west,
    left=.55 of synthesis-system.185,
    anchor=east,
] (observed-data) {Observed Dataset\\$\mt{D}=\set{(\by_i,\bx_i)}_{i=1}^{N}$};

\node[
    rectangle,
    draw=black,
    text width=2.5cm,
    minimum height=.9cm,
    align=center,
    % above=.5 of observed-data.north,
    anchor=north,
] (data-source) at (observed-data.north |- system-title.north) {Unknown Data Generating Process};

\node[
    rectangle,
    below=0 of observed-data,
    text width=2.5cm,
    align=center,
] (data-table) {
    \begin{tabular}{|l|l|l|}\hline
    $y_1$ & $y_2$ & $x_1$ \\ \hline
    1.8 & 2.1 & 4.5 \\
    3.7 & 4.2 & -2 \\
    $\cdots$ & $\cdots$ & $\cdots$ \\ \hline
    \end{tabular}
};

\node[
    rectangle,
    draw=black,
    text width=3.5cm,
    minimum height=.825cm,
    align=center,
    above left=0 and 2 of synthesis-system.center,
    anchor=south,
] (ast-prior) {Prior Distribution $\mt{A}$ over\\DSL Source Code $\mt{S}_d$};

\node[
    rectangle,
    draw=black,
    text width=3.7cm,
    minimum height=.825cm,
    align=center,
    above right=0 and 2 of synthesis-system.center,
    anchor=south,
] (code-generator) {Code Generator $\mt{G}$\\
    DSL Code $\mt{S}_d$ $\mapsto$ PPL Code $\mt{S}_p$
};

\node[
    rectangle,
    draw=black,
    text width=3.5cm,
    align=center,
    below=0.1 of ast-prior,
    minimum height=.75cm,
    anchor=north,
] (likelihood-estimator) {Program Score Estimator\\
    $P_{\mt{A}}(\mt{S}_d) \times P_{\mt{S}_p}(\mt{D})$
};

\node[
    rectangle,
    draw=black,
    text width=3.7cm,
    align=center,
    below=0.1 of code-generator,
    anchor=north,
    minimum height=.75cm,
] (program-mutations) {Stochastic Program Mutations\\
    $(\mt{S}_d, \mt{S}_p) \mapsto (\mt{S}'_d, \mt{S}'_p)$
};

\node[
    rectangle,
    draw=none,
    text width=8cm,
    align=center,
    below=.55 of synthesis-system.south,
    anchor=north,
] (sampled-program) {Ensemble of $M$ Synthesized Probabilistic Programs\\
    $\set{\mt{S}_p}$ Sampled from the Bayesian Posterior};

\node[
    rectangle,
    text width=8cm,
    below=0 of sampled-program.south,
    anchor=north,
    draw=black,
    fill=white,
    copy shadow={draw, fill=white, shadow xshift=1.5mm, shadow yshift=-1.5mm},
    copy shadow={draw, fill=white, shadow xshift=1.0mm, shadow yshift=-1.0mm},
    copy shadow={draw, fill=white, shadow xshift=0.5mm, shadow yshift=-0.5mm},
] (program-text) {
\begin{lstlisting}[style=venturescript,basicstyle=\ttfamily\tiny,]
 assume y1 = (x1) ~> {if (x1 > 0) poisson(x1) else poisson(-x1)};
 assume y2 = (y1) ~> {normal(y1, 1)};
\end{lstlisting}
};

\node[
    draw=black,
    align=center,
    text width=2.5cm,
    below right=.75 and 2.25 of program-text.south,
    anchor=north,
] (dynamic) {Probabilistic\\Inference Engine};


\node[
    draw=black,
    align=center,
    text width=2.5cm,
    below left=.75 and 2.25 of program-text.south,
    anchor=north,
] (static) {Static Code\\Analysis};

\node[
    left=.5 of static.west,
    anchor=east,
    align=center,
] (property) {Static\\Property $W$};

\node[
    right=.5 of dynamic.east,
    anchor=west,
    align=center,
] (query) {Predictive\\Query $Q$};


\node[
    draw=black,
    below=1 of static,
    text width=2.5cm,
    align=center,
] (static-oper) {Averaging};

\node[
    draw=black,
    below=1 of dynamic,
    text width=2.5cm,
    align=center,
] (dynamic-oper) {Union};

\node[
    % draw=black,
    below=.5 of static-oper,
    text width=3cm,
    align=center,
    minimum height=.8cm,
] (static-outcome) {Probability $W$ Holds for\\ Data Generating Process};

\node[
    % draw=black,
    text width=2.5cm,
    below=.5 of dynamic-oper,
    align=center,
    minimum height=.8cm,
] (dynamic-outcome) {Query Result Set\\$\cup_{i=1}^{M}\set{r_i}$};

% \node[
%     below=0.3 of dynamic,
%     text width=3cm,
%     align=center,
% ] (dynamic-text) {predictive properties of learned programs};

\draw[decorate,decoration={brace,amplitude=5pt,raise=3pt}]
    ($(program-text.south west) - (0,0.10)$) -- (program-text.north west)
    node[pos=0.5, xshift=-1cm, text width=1cm, align=center] {$M$\\Programs};

\draw[-latex] (data-source) -- (observed-data);
\draw[-latex] (observed-data.east) -- (synthesis-system.185);
\draw[-latex](synthesis-system) -- (sampled-program);

\draw[-latex]($(static.north |- program-text.south) -(0,0.05)$)
    -- ($(static.north) -(0,0)$);
\draw[-latex]($(static.north |- program-text.south) -(0.66,0.15)$)
    -- ($(static.north) -(0.66,0)$);
\draw[-latex]($(static.north |- program-text.south) +(0.66,0)$)
    -- ($(static.north) +(0.66,0)$);
\draw[-latex]($(static.north |- program-text.south) -(0.33,0.10)$)
    -- ($(static.north) -(0.33,0)$);
\draw[-latex,draw=none]($(static.north |- program-text.south) +(0.33,0)$)
    -- ($(static.north) +(0.33,0)$)
    node[fill=none,pos=.5]{...};

\draw[-latex] (static.south) -- (static-oper.north)
    node[fill=white,pos=.5]{1};
\draw[-latex]($(static.south) -(0.66,0)$) -- ($(static-oper.north) -(0.66,0)$)
    node[fill=white,pos=.5]{0};
\draw[-latex]($(static.south) +(0.66,0)$) -- ($(static-oper.north) +(0.66,0)$)
    node[fill=white,pos=.5]{0};
\draw[-latex]($(static.south) -(0.33,0)$) -- ($(static-oper.north) -(0.33,0)$)
    node[fill=white,pos=.5]{1};
\draw[-latex,draw=none]($(static.south) +(0.33,0)$) -- ($(static-oper.north) +(0.33,0)$)
    node[fill=none,pos=.5]{...};

\draw[-latex]($(dynamic.north |- program-text.south) -(0,0.05)$)
    -- ($(dynamic.north) -(0,0)$);
\draw[-latex]($(dynamic.north |- program-text.south) -(0.66,0.15)$)
    -- ($(dynamic.north) -(0.66,0)$);
\draw[-latex]($(dynamic.north |- program-text.south) +(0.66,0)$)
    -- ($(dynamic.north) +(0.66,0)$);
\draw[-latex]($(dynamic.north |- program-text.south) -(0.33,0.10)$)
    -- ($(dynamic.north) -(0.33,0)$);
\draw[-latex,draw=none]($(dynamic.north |- program-text.south) +(0.33,0)$)
    -- ($(dynamic.north) +(0.33,0)$)
    node[fill=none,pos=.5]{...};

\draw[-latex] (dynamic.south) -- (dynamic-oper.north)
    node[fill=white,pos=.5]{$r_3$};
\draw[-latex]($(dynamic.south) -(0.66,0)$) -- ($(dynamic-oper.north) -(0.66,0)$)
    node[fill=white,pos=.5]{$r_1$};
\draw[-latex]($(dynamic.south) +(0.66,0)$) -- ($(dynamic-oper.north) +(0.66,0)$)
    node[fill=white,pos=.5]{$r_M$};
\draw[-latex]($(dynamic.south) -(0.33,0)$) -- ($(dynamic-oper.north) -(0.33,0)$)
    node[fill=white,pos=.5]{$r_2$};
\draw[-latex,draw=none]($(dynamic.south) +(0.33,0)$) -- ($(dynamic-oper.north) +(0.33,0)$)
    node[fill=none,pos=.5]{...};

\draw[-latex] (property) -- (static);
\draw[-latex] (query) -- (dynamic);

\draw[-latex] (static-oper) -- (static-outcome);
\draw[-latex] (dynamic-oper) -- (dynamic-outcome);

% \draw[-latex](program-text) -- (dynamic);
% \draw[-latex](program-text) -- (static);

% \draw[-latex](dynamic) -- (dynamic-text);
% \draw[-latex](static) -- (static-text);

\end{tikzpicture}

\smallskip
\caption{Overview of Bayesian synthesis and analysis of probabilistic programs
for automatic data modeling.}
\label{fig:synthesis-overview}
\end{figure}


==> figures/gp-edits.tex <==
%!TEX root = ../paper.tex

\definecolor{EditDeleteColor}{RGB}{255,175,175}
\definecolor{EditAddColor}{RGB}{200,225,255}

\begin{figure}[!ht]
\centering
%%%%%%%%%%%%%%%%%%%%%%%%%
% constant ==> constant %
%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subfigure}{0.8\linewidth}
\begin{minipage}[t]{0.40\textwidth}
\sethlcolor{EditDeleteColor}
\begin{lstlisting}[style=dsledits, basicstyle=\ttfamily\scriptsize]
(+ (wn 0.1)
   (* (+ (wn 49.5)
         (const 25.4))
      (+ (per 13.2 8.6)
         (+ (lin (*@\hl{1.2}@*))
            (lin 4.8)))))
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.1\textwidth}
\vspace{1cm}
$\overset{\rm mutation}{\longrightarrow}$
\end{minipage}
\begin{minipage}[t]{0.55\textwidth}
\sethlcolor{EditAddColor}
\begin{lstlisting}[style=dsledits, basicstyle=\ttfamily\scriptsize]
(+ (wn 0.1)
   (* (+ (wn 49.5)
         (const 25.4))
      (+ (per 13.2 8.6)
         (+ (lin (*@\hl{1.8}@*))
            (lin 4.8)))))
\end{lstlisting}
\end{minipage}
\captionsetup{skip=0pt}
\caption{Change a single constant.}
\end{subfigure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% binary operator => binary operator %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subfigure}{0.8\linewidth}
\begin{minipage}[t]{0.40\textwidth}
\sethlcolor{EditDeleteColor}
\begin{lstlisting}[style=dsledits, basicstyle=\ttfamily\scriptsize]
(+ (wn 0.1)
   ((*@\hl{*}@*) (+ (wn 49.5)
         (const 25.4))
      (+ (per 13.2 8.6)
         (+ (lin 1.2)
            (lin 4.8)))))
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.1\textwidth}
\vspace{1cm}
$\overset{\rm mutation}{\longrightarrow}$
\end{minipage}
\begin{minipage}[t]{0.55\textwidth}
\sethlcolor{EditAddColor}
\begin{lstlisting}[style=dsledits, basicstyle=\ttfamily\scriptsize]
(+ (wn 0.1)
   ((*@\hl{+}@*) (+ (wn 49.5)
         (const 25.4))
      (+ (per 13.2 8.6)
         (+ (lin 1.2)
            (lin 4.8)))))
\end{lstlisting}
\end{minipage}
\captionsetup{skip=0pt}
\caption{Replace a binary operator with a randomly chosen binary operator.}
\end{subfigure}

%%%%%%%%%%%%%%%%%%%%%%%%
% terminal => terminal %
%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subfigure}{0.8\linewidth}
\begin{minipage}[t]{0.40\textwidth}
\sethlcolor{EditDeleteColor}
\begin{lstlisting}[style=dsledits, basicstyle=\ttfamily\scriptsize]
(+ (*@\hl{(wn 0.1)}@*)
   (* (+ (wn 49.5)
         (const 25.4))
      (+ (per 13.2 8.6)
         (+ (lin 1.2)
            (lin 4.8)))))
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.1\textwidth}
\vspace{1cm}
$\overset{\rm mutation}{\longrightarrow}$
\end{minipage}
\begin{minipage}[t]{0.55\textwidth}
\sethlcolor{EditAddColor}
\begin{lstlisting}[style=dsledits, basicstyle=\ttfamily\scriptsize]
(+ (*@\hl{(const 0.01)}@*)
   (* (+ (wn 49.5)
         (const 25.4))
      (+ (per 13.2 8.6)
         (+ (lin 1.2)
            (lin 4.8)))))
\end{lstlisting}
\end{minipage}
\captionsetup{skip=0pt}
\caption{Replace a terminal node with a randomly chosen terminal node.}
\end{subfigure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% terminal ==> non-terminal %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subfigure}{0.8\linewidth}
\begin{minipage}[t]{0.40\textwidth}
\sethlcolor{EditDeleteColor}
\begin{lstlisting}[style=dsledits, basicstyle=\ttfamily\scriptsize]
(+ (wn 0.1)
   (* (+ (wn 49.5)
         (*@\hl{(const 25.4)}@*))
      (+ (per 13.2 8.6)
         (+ (lin 1.2)
            (lin 4.8)))))
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.1\textwidth}
\vspace{1cm}
$\overset{\rm mutation}{\longrightarrow}$
\end{minipage}
\begin{minipage}[t]{0.55\textwidth}
\sethlcolor{EditAddColor}
\begin{lstlisting}[style=dsledits, basicstyle=\ttfamily\scriptsize]
(+ (wn 0.1)
   (* (+ (wn 49.5)
         (*@\hl{(+ (lin -3.1)}@*)
            (*@\hl{(cp 2.1 (lin 1.2)}@*)
                   (*@\hl{(const 3.5)))}@*))
      (+ (per 13.2 8.6)
         (+ (lin 1.2)
            (lin 4.8)))))
\end{lstlisting}
\end{minipage}
\captionsetup{skip=0pt}
\caption{Replace a terminal node with a randomly chosen non-terminal node.}
\end{subfigure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% non-terminal => terminal %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subfigure}{0.8\linewidth}
\begin{minipage}[t]{0.40\textwidth}
\sethlcolor{EditDeleteColor}
\begin{lstlisting}[style=dsledits, basicstyle=\ttfamily\scriptsize]
(+ (wn 0.1)
   (* (+ (wn 49.5)
         (const 25.4))
      (*@\hl{(+ (per 13.2 8.6)}@*)
         (*@\hl{(+ (lin 1.2)}@*)
            (*@\hl{(lin 4.8)}@*)))
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.1\textwidth}
\vspace{1cm}
$\overset{\rm mutation}{\longrightarrow}$
\end{minipage}
\begin{minipage}[t]{0.40\textwidth}
\sethlcolor{EditAddColor}
\begin{lstlisting}[style=dsledits, basicstyle=\ttfamily\scriptsize]
(+ (wn 0.1)
   (* (+ (wn 49.5)
         (const 25.4))
      (*@\hl{(wn 6.1)}@*)))
\end{lstlisting}
\end{minipage}
\captionsetup{skip=0pt}
\caption{Replace a non-terminal node with a randomly chosen terminal node.}
\end{subfigure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% non-terminal => non-terminal %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subfigure}{0.8\linewidth}
\begin{minipage}[t]{0.40\textwidth}
\sethlcolor{EditDeleteColor}
\begin{lstlisting}[style=dsledits, basicstyle=\ttfamily\scriptsize]
(+ (wn 0.1)
   (*@\hl{(* (+ (wn 49.5)}@*)
         (*@\hl{(const 25.4))}@*)
      (*@\hl{(+ (per 13.2 8.6)}@*)
         (*@\hl{(+ (lin 1.2)}@*)
            (*@\hl{(lin 4.8))))}@*))
\end{lstlisting}
\end{minipage}
\begin{minipage}[t]{0.1\textwidth}
\vspace{1cm}
$\overset{\rm mutation}{\longrightarrow}$
\end{minipage}
\begin{minipage}[t]{0.55\textwidth}
\sethlcolor{EditAddColor}
\begin{lstlisting}[style=dsledits, basicstyle=\ttfamily\scriptsize]
(+ (wn 0.1)
   (*@\hl{(cp 1.4 (const 6.4)}@*)
           (*@\hl{(+ (const 1.2)}@*)
              (*@\hl{(lin -0.4)))}@*))
\end{lstlisting}
\end{minipage}
\captionsetup{skip=0pt}
\caption{Replace a non-terminal node with a randomly chosen non-terminal node.}
\end{subfigure}

\captionsetup{skip=5pt}
\caption{Classes of mutations applied a time series DSL program during
Bayesian program synthesis.}
\label{fig:gp-edits}
\end{figure}


==> figures/gp-synthesized.tex <==
%!TEX root=../paper.tex

\begin{figure}
\centering

\includegraphics[width=\linewidth]{assets/gas-synthesized-programs-row.pdf}

% \captionsetup{skip=0pt}
\caption{Synthesized programs represent structural uncertainty in the
temporal characteristics of the underlying data. The left panel shows a time
series of gas production from 1956 to 1995. The middle and right panels show
source code of Venture programs synthesized from the posterior distribution
given the data, along with predictions from their corresponding Gaussian process
stochastic procedures. Both programs detect a change point around 1968 with a
constant kernel in the left regime. However the program in the middle panel
fits a smoothing kernel in the regime after change point, whereas the program in
the right panel fits products of linear and periodic kernels. Simulations from
both programs illustrate sensible fit to the data, despite different hypotheses
on the covariance structure and noise model.}
\end{figure}


==> technical.tex <==
%!TEX root=./paper.tex

\clearpage

\input{figures/diagram-v2}

\clearpage

\section{Bayesian Synthesis of Probabilistic Programs}
\label{sec:bayesian-probabilistic-program-synthesis}

This section provides the formal definitions behind our synthesis framework
shown in Figure~\ref{fig:synthesis-overview}, and technical details of the
implementation of the framework for two domain-specific languages.
%
The objective of probabilistic program synthesis is to learn the source code of
a probabilistic program by observing its outputs given a set of inputs
at which it was evaluated.
%
As opposed to directly synthesizing raw source code of arbitrary programs in a
\textit{probabilistic programming language} (PPL) such as Venture, our approach
is instead based on first defining a ``high-level'' \textit{domain-specific
language} (DSL) for a given application domain.
%
A DSL specifies a family of probabilistic models, and each DSL program
$\mt{S}_d$ is one member of this family.
%
A key property of DSL programs is that they are typically represented as
high-level, human-interpretable strings or data structures, as opposed to being
executable probabilistic code that implement complex algorithms using
variable assignment, procedural abstraction and control flow.

\input{figures/diagram}

The next step is to use a \textit{code generator} $\mt{G}$, which takes a DSL
program $\mt{S}_d$ and outputs probabilistic source code $\mt{S}_p$ in the PPL
that represents the generative process of the probabilistic model specified by
the DSL program.
%
The set of probabilistic programs produced by the code generator $\mt{G}$ is
typically a small subset of all possible programs that can be expressed in the
PPL.
%
This property allows us to narrow the search space of synthesis, from arbitrary
program text in the PPL, to only those probabilistic programs which have a
corresponding program in the DSL.

After having synthesized a set of PPL programs, we perform two types of program
analyses: (i) static analysis (by parsing the program text) provides insight
into probable structural properties of the learned models; and (ii)
probabilistic inference (by running the programs in a probabilistic programming
environment) provides insight into their predictive properties, such as
producing forecasts or simulations.

We embed the synthesis problem in a Bayesian inference framework. An overview of
the approach is given in Figure~\ref{fig:synthesis-overview}. The main
components of the system are:
%
\begin{enumerate}
\item Observed data $\mt{D} = \set{(\by_i, \bx_i)}_{i=1}^N$, which is a set of
$N$ observations of the output $\by_i$ assumed to be generated by an (unknown)
PPL model program $\mt{S}_d$, given input $\bx_i$.

\item Prior distribution $\mt{A}$ over DSL source code $\mt{S}_d$, which defines
a generative model $\mt{S}_d \sim P_{\mt{A}}$ over valid programs in the
domain specific language.

\item Code generator $\mt{G}$, which accepts a DSL program $\mt{S}_d$ and
produces source code of a probabilistic program $\mt{S}_p \equiv
\mt{G}(\mt{S}_d)$ in a PPL.
%
We use the symbol $P_{\mt{S}_p}(\bm{\theta}, \by_{1:N} ; \bx_{1:N})$ to denote
full joint probability distribution (or density) of the model program's trace,
which contains outputs $\by_{1:N}$, given inputs $\bx_{1:N}$. Here,
$\bm{\theta}$ is the collection of random choices made by the PPL program which
are not specified by the DSL program.

\item Program score estimator, which returns the joint probability density of
(i) random choices made by the DSL prior $\mt{A}$; (ii) random choices made by
the PPL model program $\mt{S}_p$, and (iii) the observed data $\mt{D}$. This
joint probability is given by the following expression:
%
\begin{align}
  P_{\mt{A}}(\mt{S}_d)
  \left[
    P_{\mt{S}_p}(\bm{\theta})
    \prod_{i=1}^{N} P_{\mt{S}_p}(\by_i \mid \bm{\theta}, \by_{1:i-1}; \bx_{1:i})
  \right]
  && \textrm{where } \mt{S}_p \equiv \mt{G}(\mt{S}_d).
\label{eq:synthesis-unnormalized-target}
\end{align}

\item Stochastic program mutator, which uses Bayesian inference to propose edits
$(\mt{S}_d, \mt{S}_p) \mapsto (\mt{S}'_d, \mt{S}'_p)$ to the current DSL/PPL
programs, and accepts or rejects the edits in such a way that ensures programs
are approximately sampled according to the target distribution
Eq~\eqref{eq:synthesis-unnormalized-target}.

\item Static code analyzer, which first takes a property $W$ and a set of
PPL programs $\set{\mt{S}_p}$ sampled from the posterior, then
determines whether the property holds in each program by directly parsing the
source code. The fraction of programs where $W$ holds approximates the posterior
probability of the structure existing in the data generating process.

\item Probabilistic inference engine, which takes a query $Q$ and a set of
PPL programs $\set{\mt{S}_p}$ sampled from the posterior, executes them, and
returns the prediction result $r_i$ according to each program. The union of
results $\cup\set{r_i}_{i=1}^M$ represents the posterior distribution over the
result.
\end{enumerate}

The target distribution Eq~\eqref{eq:synthesis-unnormalized-target} leads the
Bayesian synthesizer to search over the execution trace of DSL prior $\mt{A}$ to
sample probable DSL programs $\mt{S}_d$, which, when passed through the code
generator $\mt{G}$, result in PPL programs $\mt{S}_p$ that explain the observed
data $\mt{D}$ well.

In the rest of this section, we describe two instantiations of the Bayesian
synthesis framework for two domain-specific languages used throughout the paper.
The first DSL, introduced in Section~\ref{subsec:example-gp-introduction},
specifies a family of nonparametric regression models for univariate time series
data, and the second DSL specifies a family of nonparametric mixture models for
multivariate tabular data. These domain-specific languages correspond to
families of probabilistic models that can capture rich probabilistic structures
which appear frequently in each of the respective problem domains.

\subsection{A Gaussian Process DSL for Univariate Time Series}
\label{subsec:gp-synthesis}

\input{figures/gp-synthesized}

Section~\ref{subsec:example-gp-introduction} introduced the mathematical
formalism and domain-specific language for Gaussian process models. In this
section, we provide the technical details of how synthesis operates.

The DSL source code prior $\mt{A}$ (first codebox in
Figure~\ref{fig:gp-tutorial}) specifies a prior over DSL programs $\mt{S}_d$
from the grammar in Section~\ref{subsec:example-gp-introduction}, which we
represent as a binary tree. Each leaf $n$ of $\mt{S}_d$ is a pair $(k_n, h_n)$
comprised of a base kernel and its hyperparameters. The structure of $\mt{S}_d$
is encoded by the index $n$ of each internal node (whose left child is $2n$ and
right child is $2n+1$) and the operators and base kernels at each node.
%
Let $N$ denote the total number of nodes in $\mt{S}_d$. We write $\mt{S}_d =
\cup_{n=1}^{N}{\set{u_n}}$ as a collection of $N$ random variables, where $u_n =
(b_n, o_n, k_n, h_n)$ is a tuple of random variables for node $n$: $b_n$ is 1
if the tree branches at $n$ (and 0 if $n$ is a leaf); $o_n$ is the operator (or
$\varnothing$ if $b_n=0$); $k_n$ is the base kernel (or $\varnothing$ if
$b_n=1$); and $h_n$ is the hyperparameter vector (or $\varnothing$ if $n$ has no
hyperparameters, e.g., if $b_n = 1$ and $o_n = +$). Letting $\pi(n)$ denote the
list of all nodes in the path from $n$ up to the root, the DSL prior $\mt{A}$ is:
%
\begin{align}
P_{\mt{A}}(\mt{S}_d)
  &= \prod_{n=1}^{N}P_{\mt{A}}(u_n|u_{\pi(n)})
  = \prod_{n=1}^{N} \begin{cases}
  (1{-}p_\mathrm{branch})\,
    p_\mathrm{kernel}(k_n)\,
    p^k_\mathrm{hyper}(h_n\,{\mid}k_n)
    & \textrm{if}\; b_n = 0,\\
  (p_\mathrm{branch})
    p_\mathrm{oper}(o_n)
    p^o_\mathrm{hyper}(h_n\,{\mid}o_n)
  & \textrm{if}\; b_n = 1\\
  % 0
  % & \textrm{if}\; u_n|u_{\pi(n)}\; \textrm{}
\end{cases}
  \label{eq:gp-dsl-prior}
\end{align}
%
Note that Eq~\eqref{eq:gp-dsl-prior} is set to 0 for invalid tree topologies.
The distributions $p_\textrm{branch}$, $p_\textrm{kernel}$, $p_\textrm{oper}$
and $p_\mathrm{hyper}$ are all fixed constants in $\mt{A}$.

Having specified the prior for DSL code $\mt{S}_d$, we then feed it into a code
generator $\mt{G}$ which produces a PPL program in Venture $\mt{S}_p$,
with mean 0 an covariance function given by $\mt{S}_d$.
Figure~\ref{subfig:gp-tutorial-prior} shows an example DSL program and its
generated Venture PPL code.

Finally, we complete the template in Eq~\eqref{eq:synthesis-unnormalized-target}
by specifying the joint distribution of variables in the trace of $\mt{S}_p$.
This program, which has no auxiliary randomness $\bm{\theta}$, takes as input
$k$ probe points $\bx_{1:k} \in \mathbb{R}^k$, and produces as output a joint
sample $\by_{1:k} \in \mathbb{R}^k$ from the GP at the probe points:
%
\begin{align}
\log P_{\mt{S}_p}(\by_{1:k}; \bx_{1:k})
&= \log \mathcal{N}(\by_{1:k} \mid 0, \Kprior +
  \sigma^2 \mathbf{I}) \quad\quad
  (
    \mathrm{where}\; \Kprior = \left[
      \mathrm{cov}\left(y_{i}, y_{j}\right)
    \right]_{1\le i,j \le k}
  )
\notag \\
&= -\frac{1}{2} (\by_{1:k} )^\top (\Kprior + \sigma^2
  \mathbf{I})^{-1}\by_{1:k}
  - \frac{1}{2}\log \abs{\Kprior + \sigma^2 \mathbf{I}}
  - \frac{k}{2}\log 2\pi.
\label{eq:gp-ppl-liklelihood}
\end{align}

\subsubsection{Algorithms for Bayesian synthesis in the GP covariance kernel
DSL}
\label{subsubsec:gp-synthesis-inference}

The key inference problem in Eq~\eqref{eq:synthesis-unnormalized-target} is
searching over the space of (i) GP kernel compositions $o_n$, and (ii) base
kernels and their hyperparameters $(k_n,h_n)$, for each node $n$ in $\mt{S}_d$.
%
Our strategy for inference on structure is to simulate a Markov chain whose
target distribution is $p_{\mt{A}}(\mt{S}_d|\mt{D})$. The following
Metropolis-Hastings (MH) algorithm for mutating the programs is implemented by
the Venture inference expression %
\lstinline[style=venturescript]{infer resimulate(minimal_subproblem(/?structure))}
(invoked in the third code box of Figure~\ref{fig:gp-tutorial}).
%
Suppose the current DSL code is $\mt{S}_d$. We sample from the proposal
distribution $Q(\mt{S}_d \to \mt{S}'_d)$ using a three-step process. First,
select a node $u_n \in \mt{S}_d$, and let $\mt{S}^n_d$ denote the subtree of
$\mt{S}_d$ rooted at $n$. Second, ``detach'' $u_n$ and all its descendants from
$\mt{S}_d$, which gives a truncated program %
$\mt{S}_d^{\textrm{detach}} := \mt{S}_d \setminus \mt{S}^n_d$.
%
Third, ``resimulate'', starting from $\mt{S}_d^{\textrm{detach}}$, the random
choice $u'_n$ using a resimulation distribution $q(u'_n;
\mt{S}_d^{\textrm{detach}}) \equiv P_{\mt{A}}(u'_n\mid u_{\pi(n)})$ equal to the
prior Eq~\eqref{eq:gp-dsl-prior}.
%
If $b_n' = 0$ (i.e., a branch node), recursively resimulate its children until
all downstream random choices are leaf nodes. This operation results in a new
program $\mt{S}_d'^{n}$, and we set %
$\mt{S}_{d}' = \mt{S}_{d}^{\textrm{detach}} \cup \mt{S}_{d}'^{n}$ to be the
proposal.
%
To compute the reversal $Q(\mt{S}_{d}'\to\mt{S}_{d})$, we make the following key
observation: when resimulating node $u'_n$ starting from $\mt{S}_{d}'$, the
truncated programs $\mt{S}_{d}^{\mathrm{detach}} =
\mt{S}_{d}'^{\mathrm{detach}}$ are identical for $Q(\mt{S}_{d}\to\mt{S}_{d}')$ and
$Q(\mt{S}_{d}'\to\mt{S}_{d})$. Using this insight, the MH acceptance ratio is
therefore:
%
\begin{align}
&\alpha(\mt{S}_{d} \to \mt{S}_{d}')
= \frac{
   P_{\mt{A}}(\mt{S}_{d}')P_{\mt{S}'_d}(\by;\bx) Q(\mt{S}_{d}'\to\mt{S}_{d})}{
   P_{\mt{A}}(\mt{S}_{d})P_{\mt{S}_d}(\by;\bx) Q(\mt{S}_{d}\to\mt{S}'_{d})
    }
= \frac{
    \left(\prod_{n=1}^{N}P_{\mt{A}}(u'_n|u'_{\pi'(n)})\right)
    P_{\mt{S}'_p}(\by; \bx) Q(\mt{S}_{d}'\to\mt{S}_{d})
    }{
    \left(\prod_{n=1}^{N}P_{\mt{A}}(u_n|u_{\pi(n)})\right)
    P_{\mt{S}_p}(\by; \bx) Q(\mt{S}_{d}\to\mt{S}_{d}')
  } \notag \\
&= \frac{
    \left(
      \prod_{n\in{\mt{S}_{d}'^{\mathrm{detach}}}}P_{\mt{A}}(u'_n|u'_{\pi'(n)})
    \right)
    \left(
      \prod_{n\in{\mt{S}_{d}'^n}}P_{\mt{A}}(u'_n|u'_{\pi'(n)})
    \right)
      P_{\mt{S}'_p}(\by; \bx)
    \left(
      \prod_{n\in{\mt{S}_{d}^n}}P_{\mt{A}}(u_n|u_{\pi'(n)})
    \right)
    }{
    \left(
      \prod_{n\in{\mt{S}_{d}^{\mathrm{detach}}}}P_{\mt{A}}(u_n|u_{\pi(n)})
    \right)
    \left(
      \prod_{n\in{\mt{S}_{d}^n}}P_{\mt{A}}(u_n|u_{\pi(n)})
    \right)
      P_{\mt{S}_p}(\by; \bx)
    \left(
      \prod_{n\in{\mt{S}_{d}^{'n}}}P_{\mt{A}}(u'_n|u_{\pi'(n)})
    \right)
  }\notag \\
& = \frac{P_{\mt{S}'_p}(\by;\bx)}{P_{\mt{S}_p}(\by;\bx)}.
\label{eq:mh-acceptance-ratio}
\end{align}
%
Eq~\eqref{eq:mh-acceptance-ratio}, which is a likelihood ratio of terms in the
form of Eq~\eqref{eq:gp-ppl-liklelihood}, can be computed without revisiting the
entire trace \citep{mansinghka2014}. Algorithm~\ref{alg:resimulation-mh}
summarizes the key elements of the procedure.
%
Stochastic mutation of hyperparameters $\set{h_n}$ in the DSL program $\mt{S}_d$
is also based on MH inference, shown in Algorithm~\ref{alg:hypers-mh}. Both of
these algorithms are implemented using general purpose inference machinery in
Venture. Their respective inference programs are shown in the captions.

\begin{algorithm}[H]
\small
\caption{Resimulation MH for mutating the structure of the DSL program.\\
Inference program: \lstinline[style=venturescript,basicstyle=\ttfamily\footnotesize]{infer resimulate(minimal_subproblem(/?structure==pair("branch", n)))}}
\label{alg:resimulation-mh}
\begin{algorithmic}[1]
\Require{Index $n$ of node in the DSL program whose
  subtree structure $\mt{S}^n_d$ to transition.
}
\Ensure{Program mutation $\mt{S}^n_d\to\mt{S}^{'n}_d$,
  targeting $p_{\mt{A}}(\mt{S}^n_d|\mt{S}_d\setminus{\mt{S}^n_d}, \mt{D})$.
}
\State $\mt{S}_d^{\textrm{detach}} \gets \mt{S}_d \setminus \mt{S}^n_d$
  \Comment{Detach the subtree rooted at $n$.}
\State $\mt{S}_d^{'n} \sim p_{\mt{A}}(\cdot \mid \mt{S}_d^{\textrm{detach}})$
  \Comment{Resimulate the subtree rooted at $n$.}
\State $\mt{S}_d' \gets \mt{S}_d^{\textrm{detach}} \cup \mt{S}^{'n}_d$
  \Comment{Construct the proposal tree.}
\State $\alpha \gets
    {P_{\mt{S}'_p}(\by_{1:N};\bx_{1:N})}/{P_{\mt{S}_p}(\by_{1:N};\bx_{1:N})}$
  \Comment{Compute the acceptance ratio.}
\If{$\textsc{Uniform}[0,1] \le \alpha$}
  $\mt{S}^n_d \gets \mt{S}^{'n}_d$
  \Comment{Accept the proposal with probability $\alpha$.}
\EndIf
\end{algorithmic}
\end{algorithm}\vspace{-1cm}%
\begin{algorithm}[H]
\small
\caption{Resimulation MH for mutating hyperparameters of base kernels in the DSL
program.\\
Inference program: \lstinline[style=venturescript,basicstyle=\ttfamily\footnotesize]{infer resimulate(minimal_subproblem(/?hypers==n))}}
\label{alg:hypers-mh}
\begin{algorithmic}[1]
\Require{Index $n$ of node in DSL source tree whose hyperparameters to transition}
\Ensure{Program mutation $h_n \to h'_n$, targeting
  $P_{\mt{A}}(h_n | \mt{S}_d\setminus{\set{h_n}}, \mt{D}$).}
\State $h'_n \sim q(\cdot \; ; \mt{S}_d, \mt{D})$
  \Comment{Propose a new value of $h'_n$.}
\State $\mt{S}'_d \gets (\mt{S}_d \cup \set{h'_n}) \setminus \set{h_n}$
  \Comment{Construct proposal program}
\State $q_{\textrm{R}} =
  p^k_{\rm hyper}(h'_n\mid k_n)P_{\mt{S}'_p}(\by_{1:N}; \bx_{1:N})
  \, q(h_n ; \mt{S}'_d, \mt{D})$
\Comment{Compute density of reverse proposal.}
\State $q_{\textrm{F}} =
  p^k_{\rm hyper}(h_n\mid k_n)P_{\mt{S}_p}(\by_{1:N}; \bx_{1:N})
  \, q(h'_n ; \mt{S}_d, \mt{D})$
\Comment{Compute density of forward proposal.}
\State $\alpha \gets q_{\textrm{R}} / q_{\textrm{F}}$
  \Comment{Compute the acceptance ratio.}
\If{$\textsc{Uniform}[0,1] \le \alpha$}
  $\mt{S}^n_d \gets \mt{S}^{'n}_d$
  \Comment{Accept the proposal with probability $\alpha$.}
\EndIf
\end{algorithmic}
\end{algorithm}

\subsection{A Nonparametric Mixture Modeling DSL for Multivariate Tabular Data}
\label{subsec:crosscat-synthesis}

Having describe a domain-specific language for nonparametric regression in
univariate time series using Gaussian process models, this section describes a
second DSL for nonparametric mixture modeling in multivariate tabular data. The
statistical setup starts with a data table containing $C$ columns and $R$ rows;
each column $c$ represents a distinct random variable $X_c$, and each row $r$ is
a joint instantiation $\set{X_1,\dots,X_C} = \set{x_{r,1},\dots,x_{r,c}}$ of all
the $C$ random variables. Our DSL describes the joint distribution over all
cells in the data table using the ``Cross-Categorization'' model class
introduced by \citet{mansinghka2014}, which we now review briefly.

Probabilistic programs in this model class assume that the set of columns $[C]
\coloneqq \set{1,\dots,C}$ is partitioned into non-overlapping blocks
$\set{\mt{V}^k}$, where each $\mt{V}^k \subset [C]$, their union satisfy $\cup_k
\mt{V}^k = [C]$, and the pairwise intersections satisfy $\mt{V}^k \cap
\mt{V}^{l} = \varnothing$ for $k\ne l$. Within each block $\mt{V}^k$ of columns,
data in the $R$ rows are distributed according to a ``naive-Bayes'' Chinese
restaurant process (CRP) mixture model, with a concentration parameter
$\alpha_k$. Similarly to the ability of GP models to express widely varying
temporal patterns in univariate time series, this family of nonparametric
mixture models is able to express probabilistic structures with a wide set of
dependence relationships that arise in multi-modal, heteroskedastic, and
heterogeneously-typed multivariate distributions.

The grammar of the DSL is shown in
Figure~\ref{subfig:crosscat-description-dsl-grammar}. It expresses the three
structures needed to describe the joint distribution of $(X_1,\dots,X_C)$: (i)
the partition of the $C$ columns into $K$ blocks $\set{\mt{V}^k}$, which
dictates the factorization of the joint distribution; (ii) the concentration
$\alpha_k$ of the Chinese restaurant process used to partition the rows within
each block $\mt{V}_k$; and (iii) the primitive univariate distributions $M_c$,
and hyperparameters $\lambda_c$, used to model the mixture components of column
$c$. Using the notations in Figure~\ref{subfig:crosscat-description-symbols},
the DSL prior shown in Figure~\ref{subfig:crosscat-description-dsl-prior} has
joint density:
%
\begin{align}
P_{\mt{A}}(\mt{S}_d)
&= P_{\mt{A}}\left( \set{\mt{V}^k}, \set{\lambda_c},
  \set{\alpha_k} \right)
= \frac{\alpha_0^K}{\prod_{c=1}^{C}(c-1+\alpha_0)}
  \prod_{k=1}^K (\lvert\mt{V}^k\rvert-1)!
  \prod_{c=1}^{c}V_c(\lambda_c)
  \prod_{k=1}^{K}\exp(-\alpha_k).
\label{eq:crosscat-dsl-prior}
\end{align}

\input{figures/crosscat-notations}

We note that, while the hyperparameters of $\tlar{distribution}$ statements in
the DSL are randomly sampled in step 2 of
Figure~\ref{subfig:crosscat-description-dsl-prior}, the actual distribution used
for each column is assumed to be deterministic based on the statistical data
type of the column (\textsf{NIGNormal} for numerical data; \textsf{GammaPoisson}
for counts data; and \textsf{DirichletCategorical} for nominal data).

We complete the template in Eq~\eqref{eq:synthesis-unnormalized-target} by
outlining the joint distribution of all latent variables $\set{\bz^k}$ and
observations $\mt{D}$ in the trace of the synthesized probabilistic program
$\mt{S}_p \equiv \mt{G}(\mt{S}_d)$, whose generative process is given in
Figure~\ref{subfig:crosscat-description-process}. The program requires no inputs
$\bx_{1:N}$, and generates outputs $\by_{1:N}$, where each observation $\by_n =
(y_{n,1},\dots,y_{n,C})$ is itself a length-$C$ vector, with density:
%
\begin{align}
&P_{\mt{S}_p}\left(\by_{1:N}, \set{\bz^k_{1:N} \mid 1 \le k \le K}\right) \notag \\
&\quad=\prod_{k=1}^K \left[
    \frac{\alpha_k^N}{\prod_{n=1}^{N}(n-1+\alpha_k)}
    \prod_{y=1}^{\max\bz^k}\left[
      (\lvert\mt{C}_j^k\rvert-1)!
      \prod_{c\in \mt{V}^k}
      M_c\left(\set{y_{c,r} \big\vert r\in \mt{C}_j^k}; \lambda_c \right)
    \right]
  \right].
\label{eq:crosscat-ppl-liklelihood}
\end{align}

\subsubsection{Example of a synthesized probabilistic program}
We now describe an example of a probabilistic program from this model class,
synthesized given a tabular dataset of patients in a heart disease study. The
table in Figure~\ref{subfig:crosscat-synthesis-data} shows eight representative
data records. The data is characterized by heterogeneous data types (nominal and
numerical), and missing data (? symbol).

\input{figures/crosscat-tutorial}
\clearpage

\noindent The target variable of interest is \ftexttt{disease}, which is an
integer between 1 and 4 indicating the level of sickness of a patient.
%
Figure~\ref{subfig:crosscat-synthesis-code} shows the source code of a
synthesized PPL model program. The \ftexttt{variable\_to\_block\_assignment}
dictionary (line 550) maps each column name to its block assignment $z_c$ in
the column partition. A simple static analysis of the synthesized program (by
e.g. inspection of the text of the data structure) can be used to show that,
according to the program, variables in block 0, such as \ftexttt{chest-pain} and
\ftexttt{max-heart-rate}, are probably predictive of the \ftexttt{disease}
outcome. On the other hand, variables in block 1 such as
\ftexttt{sex} and \ftexttt{cholesterol} are statistically independent of the
target, and contain little to no predictive signal.

The \ftexttt{variable\_to\_distributions} dictionary (line 555) maps each column
name to the primitive distributions that make up the mixture components for that
column (memoized on integer-valued cluster indexes, $\bz^k$). Note that, for a
particular column $c$, the distributions in
\ftexttt{variable\_to\_distributions} representing each mixture component all
have identical hyperparameters $\lambda_c$. However, the predictive
distributions within component $j$ differ based on the sufficient statistics of
the observed data $\set{y_{r,c} \mid z^{v_c}=j}$ assigned to that cluster in the
trace of the synthesized program \citep{murphy2007}. This feature ensures that
the mixture components specify distinct probability distributions.

The \ftexttt{block\_to\_mixture\_weights} dictionary (line 567) maps each block
in the column partition to the mixture weights of each cluster (i.e. CRP table)
within that block. The mixture models in block 0 have five modes, whereas the
mixture models in block 1 have three modes.

The \ftexttt{get\_row\_mixture\_assignment} stochastic procedure (line 570)
takes a row index and block index, and samples (according to the weights) a
cluster assignment for that row within the given block.

Finally, \ftexttt{get\_cell\_value} (line 572) is the stochastic procedure used
to simulate a value for a cell in the table. It takes a row index and a variable
name; finds the block assignment of the variable; samples a cluster assignment
within that block; and, finally, simulates a value from the distribution that
represents the sampled cluster of the queried variable.

Figure~\ref{subfig:crosscat-synthesis-analysis} shows probabilistic inference on
the trace of the synthesized program, by running it in the Venture probabilistic
programming system to obtain predictions. For a new patient record
(\ftexttt{id\_new\_patient}, line 578), we \ftexttt{observe} their
\ftexttt{chest-pain} and \ftexttt{cholesterol} values to be 2 and 160,
respectively (line 579-580). We then run 10 steps of MH inference within the
blocks of these two variables to sample probable values of this patient's
cluster assignment given the partial observations (lines 581-582). Finally, we
use the \ftexttt{predict} directive (line 583) to generate one predictive
simulation for each of the patient's
\ftexttt{thal}, \ftexttt{age}, and \ftexttt{disease} variables. The sample is
shown as a three-element list in the last line.

\subsubsection{Overview of Bayesian synthesis in the multivariate mixture
modeling DSL}
\label{subsubsec:crosscat-synthesis-inference}

We now briefly describe the strategy for Bayesian synthesis in the DSL by
outlining the mutations to each of the DSL and PPL programs. These mutations
correspond to a sequence of kernels in a Gibbs sampling MCMC routine that
targets Eqs~\eqref{eq:crosscat-dsl-prior} and
\eqref{eq:crosscat-ppl-liklelihood}. Mutations to the DSL program are:
%
\begin{enumerate}
\item For each column $c$, propose changing its block assignment $v_c$
in the column partition to another existing block, a fresh block, or keep it in
the same block.

\item For each column $c$, propose updating the hyperparameters $\lambda_c$
from a data-dependent discretization of the hyperprior $V_c$.
\item For each block $k$, propose updating the CRP concentration parameter
$\alpha_k$ from a log-space discretization of the $\mathsf{Gamma(1,1)}$
distribution.
\end{enumerate}
%
Mutations applied to the trace of PPL program are:
%
\begin{enumerate}
\item For each block $k$, and for each row $r$, propose migrating the
block assignment $z^k_r$ in the row partition to another existing block, a fresh
block, or keep it in the same block.
\end{enumerate}
%
Bayesian synthesis corresponds to cycling iteratively through the above
mutations, which results in a set of (approximately) sampled programs from the
posterior. A detailed technical description of the Gibbs sampling steps defined
above is given in \citet[Section~2.4]{mansinghka2016}.

